On the choice of proper outlet boundary conditions for numerical simulation of cardiovascular flows

It is well known that in the computational fluid dynamics simulations related to the cardiovascular system the enforcement of outflow boundary conditions is a crucial point. In fact, they highly affect the computed flow and a wrong setup could lead to unphysical results. In this chapter we discuss the main features of two different ways for the estimation of proper outlet boundary conditions in the context of hemodynamics simulations: on one side, a lumped parameter model of the downstream circulation and, on the other one, a technique based on optimal control.

==> references.tex <==
%%%%%%%%%%%%%%%%%%%%%%%% referenc.tex %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% sample references
% %
% Use this file as a template for your own input.
%
%%%%%%%%%%%%%%%%%%%%%%%% Springer-Verlag %%%%%%%%%%%%%%%%%%%%%%%%%%
%
% BibTeX users please use
% \bibliographystyle{}
% \bibliography{}
%
%\biblstarthook{

\begin{comment}
\section{Styling of References}
References may be \textit{cited} in the text either by number (preferred) or by author/year.\footnote{Make sure that all references from the list are cited in the text. Those not cited should be moved to a separate \textit{Further Reading} section or chapter.} If the citatiion in the text is numbered, the reference list should be arranged in ascending order. If the citation in the text is author/year, the reference list should be \textit{sorted} alphabetically and if there are several works by the same author, the following order should be used:
\begin{enumerate}
\item all works by the author alone, ordered chronologically by year of publication
\item all works by the author with a coauthor, ordered alphabetically by coauthor
\item all works by the author with several coauthors, ordered chronologically by year of publication.
\end{enumerate}
The \textit{styling} of references\footnote{Always use the standard abbreviation of a journal's name according to the ISSN \textit{List of Title Word Abbreviations}, see \url{http://www.issn.org/en/node/344}} depends on the subject of your book:
\begin{itemize}
\item The \textit{two} recommended styles for references in books on \textit{mathematical, physical, statistical and computer sciences} are depicted in ~\cite{science-contrib, science-online, science-mono, science-journal, science-DOI} and ~\cite{phys-online, phys-mono, phys-journal, phys-DOI, phys-contrib}.
\item Examples of the most commonly used reference style in books on \textit{Psychology, Social Sciences} are~\cite{psysoc-mono, psysoc-online,psysoc-journal, psysoc-contrib, psysoc-DOI}.
\item Examples for references in books on \textit{Humanities, Linguistics, Philosophy} are~\cite{humlinphil-journal, humlinphil-contrib, humlinphil-mono, humlinphil-online, humlinphil-DOI}.
\item Examples of the basic Springer Nature style used in publications on a wide range of subjects such as \textit{Computer Science, Economics, Engineering, Geosciences, Life Sciences, Medicine, Biomedicine} are ~\cite{basic-contrib, basic-online, basic-journal, basic-DOI, basic-mono}. 
\end{itemize}
%}
\end{comment}

\begin{thebibliography}{99.}%
% and use \bibitem to create references.
%
% Use the following syntax and markup for your references if 
% the subject of your book is from the field 
% "Mathematics, Physics, Statistics, Computer Science"
%
% Contribution 
\bibitem{Siena:2024}
P. Siena, P. C. Africa, M. Girfoglio, and G. Rozza. Chapter Six - On the accuracy and efficiency of reduced order models: Towards real-world applications. \textit{Advances in Applied Mechanics}, volume 59, pages 245-288, 2024.


\bibitem{Morbiducci:2010}
U. Morbiducci, D. Gallo, D. Massai, F. Consolo, R. Ponzini, L. Antiga, C. Bignardi, M. A. Deriu, A. Redaelli. Outflow conditions for image-based hemodynamic models of the carotid bifurcation: implications for indicators of abnormal flow. \textit{Journal of Biomechanical Engineering}, 132(9): 091005-1–091005-11, 2010.

\bibitem{Van:2011}
A. G. Van der Giessen, H. C. Groen, P. A. Doriot, P. J de Feyter, A. F. W van der Steen, F. N van de Vosse, J. J Wentzel, F. J. H Gijsen. The influence of boundary conditions on wall shear stress distribution in patients specific coronary trees. \textit{Journal of Biomechanics}, 44(6): 1089-1095, 2011.

\bibitem{Pedley:1980}
T. J. Pedley. The fluid mechanics of large blood vessels. \textit{Cambridge: Cambridge University Press}, 1980.

\bibitem{Sankaran:2012}
S. Sankaran, M. E. Moghadam, A. E. Kahn, E. E. Tseng, J. M. Guccione, A. L. Marsden. Patient-specific multiscale modeling of blood flow for coronary artery bypass graft surgery. \textit{Annals of Biomedical Engineering}, 40(10): 2228-2242, 2012.

\bibitem{Grinberg:2008}
L. Grinberg, G. E. Karniadakis. Outflow boundary conditions for arterial networks with multiple outlets. \textit{Annals of Biomedical Engineering}, 36(9): 1496-1514, 2008.

\bibitem{Zakia:2021}
Z. Zainib, F. Ballarin, S. Fremes, P. Triverio, L. Jim\'{e}nez-Juan, and G. Rozza. Reduced order methods for parametric optimal flow control in coronary bypass grafts, toward patient-specific data assimilation. \textit{International Journal for Numerical Methods in Biomedical Engineering}, 37(12):Paper No. e3367, 24, 2021.

\bibitem{Fevola:2021}
E. Fevola, F. Ballarin, L. Jim\'{e}nez-Juan, S. Fremes, S. Grivet-Talocia, G. Rozza, and 
P. Triverio. An optimal control approach to determine resistance-type boundary conditions from in-vivo data for cardiovascular simulations. \textit{International Journal for Numerical Methods in Biomedical Engineering}, 37(10):e3516, 2021.

\bibitem{Shi:2011}
Y. Shi, P. Lawford, and R. Hose. Review of zero-d and 1-d models of blood flow in the cardiovascular system. \textit{Biomedical engineering online}, 10:33, 2011.

\bibitem{Westerhof:2008}
N. Westerhof, J. W. Lankhaar, and B. Westerhof. The arterial Windkessel. \textit{Medical \& biological engineering \& computing}. 47:131–41, 2008.

\bibitem{Nichols:2022}
W. W. Nichols, M. O'Rourke, E. R. Edelman, and C. Vlachopoulos. McDonald’s blood flow in arteries: theoretical, experimental and clinical principles.  
\textit{CRC Press}, 2022.

\bibitem{Bewley:2001} T. R. Bewley. Flow control: new challenges for a new renaissance. \textit{Progress in Aerospace
sciences}, 37(1):21–58, 2001.

\bibitem{Hak:2003} 
M. Gad-el Hak, A. Pollard, and J. P. Bonnet. Flow control: fundamentals and practices, volume 53. \textit{Springer Science \& Business Media}, 2003. 

\bibitem{Gunzburger:2003} M. D. Gunzburger. \textit{Perspectives in flow control and optimization}, volume 5 of \textit{Advances
in Design and Control}, Society for Industrial and Applied Mathematics (SIAM), Philadelphia, PA, 2003. 


\bibitem{Quarteroni:2014}
A. Quarteroni. Numerical models for differential problems, volume 8 of MS\&A. \textit{Modeling, Simulation and Applications}, Springer, Milan, 2014.

\bibitem{Quarteroni:2009}
A. Quarteroni, S. Quarteroni. Numerical Models for Differential Problems. Vol 2. Milan: \textit{Springer}, 2009.

\bibitem{Girfoglio:2021}
M. Girfoglio, L. Scandurra, F. Ballarin, G. Infantino, F. Nicolo, A. Montalto, G. Rozza,
R. Scrofani, M. Comisso, and F. Musumeci. Non-intrusive data-driven rom framework for
hemodynamics problems. \textit{Acta mechanica sinica}, 37(7):1183–1191, 2021.

\bibitem{Girfoglio:2020}
M. Girfoglio, F. Ballarin, G. Infantino, F. Nicolo, A. Montalto, G. Rozza, R. Scrofani,  M. Comisso, and F. Musumeci. Non-intrusive PODI-ROM for patient-specific aortic blood flow
in presence of a LVAD device. \textit{Medical Engineering \& Physics}, 107, 103849, 2022.


\bibitem{Balzotti:2022}
C. Balzotti, P. Siena, M. Girfoglio, A. Quaini, and G. Rozza.
A data-driven reduced order method for parametric optimal blood flow control: Application to coronary bypass graft. In: \textit{Communications in Optimization Theory}, 26, 1–19, 2022.

\bibitem{Siena:2023}
P. Siena, M. Girfoglio, F. Ballarin, G. Razza. Data-Driven Reduced Order Modelling for Patient-Specific Hemodynamics of Coronary Artery Bypass Grafts with Physical and Geometrical Parameters. \textit{Journal of Scientific Computing}, 94, 38, 2023. 


\bibitem{Laskey:1990}
W. Laskey, H. Parker, V. Ferrari, W. Kussmaul, A. Noordergraaf. Estimation of total systemic arterial compliance in humans. \textit{Journal of Applied Physiology}, 1990;69: 112–9, 1990.

\bibitem{Bulpitt:1999}
C. Bulpitt, J. Cameron, C. Rajkumar, S. Armstrong, M. Connor, J. Joshi, D. Lyons, O. Moioli, P. Nihoyannopoulos. The effect of age on vascular compliance in man: Which are the appropriate measures? \textit{Journal of Human Hypertension} 1999;13: 753–8.

\bibitem{Weller:1988}
H. G. Weller, G. Tabor, H. Jasak; C. Fureby. A tensorial approach to computational continuum mechanics using object-oriented techniques.\textit{ Computers in Physics}, 12, 620–631, 1998.

\bibitem{Alnaes:2015}
M. Aln\ae{s}, J. Blechta, J. Hake, A. Johansson, B. Kehlet, A. Logg, C. Richardson, J. Ring, M. E. Rognes, and G. N. Wells. The fenics project version 1.5. \textit{Archive of Numerical
Software}, 3(100), 2015.

\bibitem{Logg:2012}
A. Logg, K. A. Mardal, and G. N. Wells, editors. Automated solution of differential equations by the finite element method, volume 84 of \textit{Lecture Notes in Computational Science and Engineering}, Springer, Heidelberg, 2012. The FEniCS book.


\bibitem{Schulz:2009}
V. Schulz and I. Gherman. One-shot methods for aerodynamic shape optimization. \textit{In MEGADESIGN and MegaOpt-German Initiatives for Aerodynamic Simulation and Optimization in Aircraft Design}, pages 207–220. Springer, 2009.

\bibitem{Ballarin:2020}
S. Ali, F. Ballarin, and G. Rozza. Stabilized reduced basis methods for parametrized steady Stokes and Navier-Stokes equations. \textit{Computers \& Mathematics with Applications}, An International Journal, 80(11):2399–2416, 2020.

\bibitem{Ballarin:2015}
F. Ballarin, A. Manzoni, A. Quarteroni, and G. Rozza. Supremizer stabilization of POD-Galerkin approximation of parametrized steady incompressible Navier-Stokes equations. \textit{International Journal for Numerical Methods in Engineering}, 102(5):1136–1161, 2015.


\end{thebibliography}

